A Hitchhiker's Guide to Geometric GNNs for 3D Atomic Systems

Recent advances in computational modelling of atomic systems, spanning molecules, proteins, and materials, represent them as geometric graphs with atoms embedded as nodes in 3D Euclidean space. In these graphs, the geometric attributes transform according to the inherent physical symmetries of 3D atomic systems, including rotations and translations in Euclidean space, as well as node permutations. In recent years, Geometric Graph Neural Networks have emerged as the preferred machine learning architecture powering applications ranging from protein structure prediction to molecular simulations and material generation. Their specificity lies in the inductive biases they leverage - such as physical symmetries and chemical properties - to learn informative representations of these geometric graphs. In this opinionated paper, we provide a comprehensive and self-contained overview of the field of Geometric GNNs for 3D atomic systems. We cover fundamental background material and introduce a pedagogical taxonomy of Geometric GNN architectures: (1) invariant networks, (2) equivariant networks in Cartesian basis, (3) equivariant networks in spherical basis, and (4) unconstrained networks. Additionally, we outline key datasets and application areas and suggest future research directions. The objective of this work is to present a structured perspective on the field, making it accessible to newcomers and aiding practitioners in gaining an intuition for its mathematical abstractions.

==> tex/conclusion.tex <==
% \section{Conclusion}

% This opinionated survey aims to provide both newcomers and experienced researchers with a pedagogical understanding of Geometric Graph Neural Networks for 3D atomic systems. 
% Throughout its course, we delve into the foundations, motivations, and distinctive features that set Geometric GNNs apart from traditional GNNs. 
% We hope that this survey provides readers with details and insights into the various steps of the Geometric GNN modelling pipeline. 
% We propose a novel taxonomy that categorizes methods into invariant, equivariant with Cartesian basis, equivariant with spherical basis, and unconstrained approaches. 
% Then, we explore a wide range of captivating applications and highlight the potential impact of Geometric GNNs in fields such as property prediction and generative modelling. 
% By showcasing their capabilities and alignment with real-world challenges, we hope to inspire further exploration and innovation in the field. 
% As we conclude our survey, we reflect on the promising research directions that lie ahead and that we believe worthy of interest, aiming to foster continued exploration and collaboration to push the boundaries of Geometric GNNs. 

% Our ultimate aspiration is to contribute to the organization and advancement of this emerging field, while igniting the curiosity of newcomers to embark on their own journey into the captivating world of Geometric GNNs. 
% By combining scholarly rigor with a comprehensive overview, we aspire to make this survey the natural go-to paper for the Geometric GNN community, facilitating knowledge dissemination and fostering future advancements.
